On the approximation of the canard explosion point in epsilon-free systems

A canard explosion is the dramatic change of period and amplitude of a limit cycle of a system of non-linear ODEs in a very narrow interval of the bifurcation parameter. It occurs in slow-fast systems and is well understood in singular perturbation problems where a small parameter epsilon defines the time scale separation. We present an iterative algorithm for the determination of the canard explosion point which can be applied for a general slow-fast system without an explicit small parameter. We also present assumptions under which the algorithm gives accurate estimates of the canard explosion point. Finally, we apply the algorithm to the van der Pol equations and a Templator model for a self-replicating system with no explicit small parameter and obtain very good agreement with results from numerical simulations.

==> texdef.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%               Newcommands              %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\im}{\textit{i}}
\newcommand{\real}{\textrm{Re}\,}
\newcommand{\imag}{\textrm{Im}\,}
\newcommand{\tr}{\textrm{tr}\,}
\newcommand{\be}{\begin{eqnarray}}
\newcommand{\ee}{\end{eqnarray}}
\newcommand{\ba}{\begin{align}}
\newcommand{\ea}{\end{align}}
\newcommand{\bi}{\begin{itemize}}
\newcommand{\ei}{\end{itemize}}
\newcommand{\du}[1]{\underline{\underline{#1}}}
\newcommand{\mt}[1]{\mathrm{#1}}
\newcommand{\nn}{\nonumber}
\newcommand{\lra}{\Leftrightarrow}
\newcommand{\linie}{\underline{\makebox[\textwidth]{}}}
\newcommand{\spacer}{\rule[-2mm]{0mm}{6mm}}
\newcommand{\notop}{{{}_{}}}
\newcommand{\ontop}[1]{{{#1}_{}}}
\newcommand{\nm}{{\rm nm\/}}
% MATH CONSTANTS


\newcommand{\kZ}{\mathcal Z}
\newcommand{\kL}{\mathcal L}
\newcommand{\kO}{\mathcal O}
\newcommand{\kB}{\mathcal B}
\newcommand{\kS}{\mathcal S}
\newcommand{\kV}{\mathcal V}
\newcommand{\kU}{\mathcal U}
\newcommand{\kW}{\mathcal W}

\newcommand{\N}{\mathbb N}
\newcommand{\C}{\mathbb C}
\newcommand{\Q}{\mathbb Q}
\newcommand{\R}{\mathbb R}
\newcommand{\Z}{\mathbb Z}
\newcommand{\bfGamma}{\mbox{$\Gamma$\hspace*{-0.6em}$\Gamma$}}
\newcommand{\bfnabla}{\makebox{\boldmath $\nabla$}}
\newcommand{\twopicubed}{(2\pi)^3}
\newcommand{\dktwopicubed}{\frac{d\kkk}{\twopicubed}}
\newcommand{\domegatwopi}{\frac{d\omega}{2\pi}}
\newcommand{\sgn}{{\rm sgn}}
\newcommand{\sm}{\!-\!}
\newcommand{\sP}{\!+\!}
\newcommand{\ve}{\varepsilon}
%\newcommand{\im}{\mathrm{Im}{}}%\newcommand{\re}{\mathrm{Re}{}}
\newcommand{\Vh}{\hat{V}}
\newcommand{\Uh}{\hat{U}}
\newcommand{\Wh}{\hat{W}}
\newcommand{\Ph}{\hat{P}}
\newcommand{\ph}{\hat{p}}
\newcommand{\pph}{\hat{\ppp}}
\newcommand{\Hh}{\hat{H}}
\newcommand{\Ad}{A^\dagger}
\newcommand{\Ah}{\hat{A}}
\newcommand{\Ahd}{\hat{A}^\dagger}
\newcommand{\Ahno}{\hat{A}^\notop}
\newcommand{\Ano}{A^\notop}
\newcommand{\cno}{c^\notop}
\newcommand{\gno}{g^\notop}
\newcommand{\Hno}{H^\notop}
\newcommand{\kno}{k^\notop}
\newcommand{\nno}{n^\notop}
\newcommand{\Nno}{N^\notop}
\newcommand{\mno}{m^\notop}
\newcommand{\pno}{p^\notop}
\newcommand{\tno}{t^\notop}
\newcommand{\uno}{u^\notop}
\newcommand{\vno}{v^\notop}
\newcommand{\Vno}{V^\notop}
\newcommand{\tauno}{\tau^\notop}
\newcommand{\lamno}{\lambda^\notop}
\newcommand{\nun}{\nu^\notop}
\newcommand{\uuu}{\mathbf{u}}
\newcommand{\uun}{\uuu^\notop}
\newcommand{\rrr}{\mathbf{r}}
\newcommand{\rrn}{\rrr^\notop}
\newcommand{\LLL}{\mathbf{L}}
\newcommand{\LLn}{\LLL^\notop}
\newcommand{\LLh}{\hat{\LLL}}
\newcommand{\PPP}{\mathbf{P}}
\newcommand{\QQQ}{\mathbf{Q}}
\newcommand{\PPn}{\PPP^\notop}
\newcommand{\RRR}{\mathbf{R}}
\newcommand{\RRn}{\RRR^\notop}
\newcommand{\kkk}{\mathbf{k}}
\newcommand{\kkn}{\kkk^\notop}
\newcommand{\qqq}{\mathbf{q}}
\newcommand{\qqn}{\qqq^\notop}
\newcommand{\ppp}{\mathbf{p}}
\newcommand{\ppn}{\ppp^\notop}
\newcommand{\sss}{\mathbf{s}}
\newcommand{\ssn}{\sss^\notop}
\newcommand{\ffn}{f^\notop}
\newcommand{\vvv}{\mathbf{v}}
\newcommand{\EEE}{\mathbf{E}}
\newcommand{\DDD}{\mathbf{D}}
\newcommand{\eee}{\mathbf{e}}
\newcommand{\een}{\mathbf{e}^\notop}
\newcommand{\GGG}{\mathbf{G}^\notop}
\newcommand{\aaa}{\mathbf{a}^\notop}
\newcommand{\bbb}{\mathbf{b}^\notop}
\newcommand{\BBB}{\mathbf{B}}
\newcommand{\AAA}{\mathbf{A}}
\newcommand{\JJJ}{\mathbf{J}}
\newcommand{\JJJp}{\mathbf{J}^{\nabla}}
\newcommand{\JJJd}{\mathbf{J}^A}
\newcommand{\krondel}[2]{\delta^\notop_{#1,#2}}
% GREEN'S FUNCTIONS
\newcommand{\nullavr}[1]{\big\langle #1 \big\rangle^\notop_{0}}
\newcommand{\eqavr}[1]{\big\langle #1 \big\rangle^\notop_{\rm eq}}
\newcommand{\impavr}[1]{\langle #1 \rangle^\notop_{\rm imp}}
\newcommand{\partau}[1]{\partial^\notop_{\tau_{#1}}}
\newcommand{\DDRPA}{{\cal D}^{\rm RPA}}
\newcommand{\DDO}{{\cal D}^{0_{}}}
\newcommand{\DD}{{\cal D}}
\newcommand{\DDn}{{\cal D}^\notop}
\newcommand{\GGO}{{\cal G}^{0_{}}}
\newcommand{\GGOs}{{\cal G}^{0_{}}_\sigma}
\newcommand{\GG}{{\cal G}}
\newcommand{\GGn}{{\cal G}^\notop}
\newcommand{\GGs}{{\cal G}^\notop_\sigma}
\newcommand{\GGb}{\bar{\cal G}^\notop}
\newcommand{\GGbO}{\bar{\cal G}^{0_{}}}
\newcommand{\Gimpk}{\impavr{\GG_\kkk}}
\newcommand{\sgm}{\sigma^\notop}
\newcommand{\Sgm}{\Sigma^\notop}
\newcommand{\SfBA}{\Sigma^{{\rm 1BA}_{}}}
\newcommand{\GfBA}{\GG^{{\rm 1BA}_{}}}
\newcommand{\AfBA}{{\cal A}^{{\rm 1BA}_{}}}
\newcommand{\GRfBA}{G^{{\rm R,1BA}_{}}}
\newcommand{\ARfBA}{A^{{\rm 1BA}_{}}}
\newcommand{\SFBA}{\Sigma^{{\rm FBA}_{}}}
\newcommand{\GFBA}{\GG^{{\rm FBA}_{}}}
\newcommand{\GSCBA}{\GG^{{\rm SCBA}_{}}}
\newcommand{\SSCBA}{\Sigma^{{\rm SCBA}_{}}}
\newcommand{\PiRPA}{\Pi^{{\rm RPA}_{}}}
\newcommand{\PiO}{\Pi^{{0}_{}}}
\newcommand{\WRPA}{W^{{\rm RPA}_{}}}
\newcommand{\SRPA}{\Sigma^{{\rm RPA}_{}}}
\newcommand{\GGm}{\bar{\bar{\mbox{$\cal G$}}}}
\newcommand{\VVm}{\bar{\bar{\mbox{$V$}}}}
\newcommand{\EEm}{\bar{\bar{\mbox{$E$}}}}
\newcommand{\IDm}{\bar{\bar{\mbox{$1$}}}}
\newcommand{\Ttau}{T^\notop_{\tau}}
\newcommand{\Tt}{T^\notop_t}
\newcommand{\Tc}{T^\notop_c}
\newcommand{\Tr}{\rm Tr}
\newcommand{\iok}{i\omega^\notop_k}
\newcommand{\ion}{i\omega^\notop_n}
\newcommand{\ikn}{ik^\notop_n}
\newcommand{\ipn}{ip^\notop_n}
\newcommand{\iqn}{iq^\notop_n}
\newcommand{\omn}{\omega^\notop_n}
\newcommand{\knn}{k^\notop_n}
\newcommand{\omnsq}{\omega^{2_{}}_n}
\newcommand{\Nimp}{N^\notop_{\rm imp}}
\newcommand{\nimp}{n^\notop_{\rm imp}}
\newcommand{\nel}{n^\notop_{\rm el}}
\newcommand{\VeffO}{V^0_{\rm eff}}
\newcommand{\VeffRPA}{V^{\rm RPA}_{\rm eff}}
% PHYSICS SYMBOLS
\newcommand{\lphi}{l_\varphi}
\newcommand{\vol}{{\cal V}}
\newcommand{\ad}{a^{\dagger}}
\newcommand{\bd}{b^{\dagger}}
\newcommand{\cd}{c^{\dagger}}
\newcommand{\aA}{a^\notop}
\newcommand{\bb}{b^\notop}
\newcommand{\cc}{c^\notop}
\newcommand{\aah}{\hat{a}^{\notop}}
\newcommand{\bbh}{\hat{b}^{\notop}}
\newcommand{\cch}{\hat{c}^{\notop}}
\newcommand{\adh}{\hat{a}^{\dagger}}
\newcommand{\bdh}{\hat{b}^{\dagger}}
\newcommand{\cdh}{\hat{c}^{\dagger}}
\newcommand{\at}{\tilde{a}}
\newcommand{\kt}{\tilde{k}}
\newcommand{\jt}{\tilde{j}}
\newcommand{\rt}{\tilde{r}}
\newcommand{\pt}{\tilde{p}}
\newcommand{\qt}{\tilde{q}}
\newcommand{\phiext}{\phi_{\rm ext}}
\newcommand{\phiind}{\phi_{\rm ind}}
\newcommand{\phitot}{\phi_{\rm tot}}
\newcommand{\chiR}{\chi^R}
\newcommand{\chiO}{\chi^\notop_0}
\newcommand{\chiOR}{\chi^{R_{}}_0}
\newcommand{\chiirr}{\chi^{\rm irr}}
\newcommand{\chiRPA}{\chi^{\rm RPA}}
\newcommand{\epsRPA}{\ve^{\rm RPA}}
\newcommand{\atd}{\at^{\dagger}}
\newcommand{\psiO}{\psi^\notop_0}
\newcommand{\psipO}{\psi^{'_{}}}
\newcommand{\psin}{\psi^\notop}
\newcommand{\psit}{\tilde{\psi}^\notop}
\newcommand{\psitd}{\psit^{\dagger}}
\newcommand{\psih}{\hat{\psi}^\notop}
\newcommand{\psidh}{\hat{\psi}^{\dagger}}
\newcommand{\Psid}{\Psi^{\dagger}}
\newcommand{\Psia}{\Psi^\notop}
\newcommand{\Psidh}{\hat{\Psi}^{\dagger}}
\newcommand{\Psiah}{\hat{\Psi}^\notop}
\newcommand{\RL}{{\rm RL}}
\newcommand{\BZ}{{\rm FBZ}}
\newcommand{\FS}{{\rm FS}}
\newcommand{\eF}{{\varepsilon^\notop_{\rm F}}}
\newcommand{\nF}{{n^\notop_{\rm F}}}
\newcommand{\nB}{{n^\notop_{\rm B}}}
%\newcommand{\kB}{{k^\notop_{\rm B}}}
\newcommand{\kF}{{k^\notop_{\rm F}}}
\newcommand{\kFsq}{{k^{2_{}}_{\rm F}}}
\newcommand{\kFcu}{{k^{3_{}}_{\rm F}}}
\newcommand{\kFpow}[1]{{k^{{#1}_{}}_{\rm F}}}
\newcommand{\lF}{{\lambda^\notop_{\rm F}}}
\newcommand{\vF}{{v^\notop_{\rm F}}}
\newcommand{\vFsq}{{v^{2_{}}_{\rm F}}}
\newcommand{\TE}{{T^\notop_{\rm E}}}
\newcommand{\TD}{{T^\notop_{\rm D}}}
\newcommand{\kD}{{k^\notop_{\rm D}}}
\newcommand{\vD}{{v^\notop_{\rm D}}}
\newcommand{\oD}{{\omega^\notop_{\rm D}}}
\newcommand{\ven}{\ve^\notop}
\newcommand{\xin}{\xi^\notop}
\newcommand{\rhoe}{\rho^\notop_{\rm el}}
\newcommand{\rhoi}{\rho^\notop_{\rm ion}}
\newcommand{\drhoi}{\delta\rho^\notop_{\rm ion}}
\newcommand{\drho}{\delta\rho}
\newcommand{\rhoiO}{\rho^\ontop{0}_{\rm ion}}
\newcommand{\omg}{\omega^\notop}
\newcommand{\oomg}{\omega^{2_{}}}
\newcommand{\spu}{{\uparrow}}
\newcommand{\spd}{{\downarrow}}
\newcommand{\aB}{{a^\notop_0}}
\newcommand{\aZ}{{a^\notop_Z}}
\newcommand{\aZsq}{{a^{2_{}}_Z}}
\newcommand{\aZcu}{{a^{3_{}}_Z}}
\newcommand{\muO}{\mu_0}
\newcommand{\eO}{e^\notop_0}
\newcommand{\eeO}{e^\ontop{2}_0}
\newcommand{\epsO}{\epsilon^\notop_0}
\newcommand{\epss}{\epsilon^{*_{}}}
\newcommand{\epsl}{{\bm{\epsilon}^\notop_\lambda}}
\newcommand{\epsv}[1]{{\bm{\epsilon}^\notop_{#1}}}
\newcommand{\vs}{v^\notop_s}
% DIRAC NOTATION
\newcommand{\bra}[1]{\langle #1 |}
\newcommand{\ket}[1]{|#1\rangle}
\newcommand{\braket}[2]{\langle #1 | #2 \rangle}
% MATH STYLE
\newcommand{\scap}{\!\cdot\!}
\newcommand{\intd}[1]{{\int\!d#1\: }}
\newcommand{\inttau}[1]{{\int_0^\beta\!d\tauno_{#1}\: }}
\newcommand{\bm}[1]{\makebox{\boldmath $#1$}}
\newcommand{\dpst}{\displaystyle}
\newcommand{\scst}{\scriptstyle}
\newcommand{\scscst}{\scriptscriptstyle}
% EQUATIONS
\newcommand{\beq}[1]{\begin{equation} \label{#1}}
\newcommand{\eeq}{\end{equation}}
\newcommand{\beqa}{\begin{eqnarray}}
\newcommand{\eeqa}{\end{eqnarray}}
\newcommand{\bal}{\begin{align}}
\newcommand{\eal}{\end{align}}
\newcommand{\bsub}{\begin{subequations}}
\newcommand{\esub}{\end{subequations}}
% \newcommand{\eqlab}[1]{\label{eq:#1}}
\renewcommand{\eqref}[1]{(\ref{eq:#1})}
\newcommand{\eqsref}[2]{(\ref{eq:#1}) and~(\ref{eq:#2})}
\newcommand{\eqsrefthree}[3]{Eqs.~(\ref{eq:#1}),~(\ref{eq:#2}),~and~(\ref{eq:#3})}
\newcommand{\exref}[1]{\ref{ex:#1}}
\newcommand{\exlab}[1]{\label{ex:#1}}
\newcommand{\figref}[1]{Fig.~\ref{fig:#1}}
\newcommand{\figlab}[1]{\label{fig:#1}}
\newcommand{\chapref}[1]{Chap.~\ref{sec:#1}}
\newcommand{\chaplab}[1]{\label{sec:#1}}
\newcommand{\secref}[1]{section~\ref{sec:#1}}
\newcommand{\seclab}[1]{\label{sec:#1}}
\newcommand{\defnref}[1]{Definition~\ref{definition:#1}}
\newcommand{\defnlab}[1]{\label{definition:#1}}
\newcommand{\exmref}[1]{Example~\ref{example:#1}}
\newcommand{\exmlab}[1]{\label{example:#1}}
\newcommand{\remref}[1]{Remark~\ref{remark:#1}}
\newcommand{\remlab}[1]{\label{remark:#1}}
\newcommand{\corref}[1]{Corollary~\ref{Corollary:#1}}
\newcommand{\corlab}[1]{\label{Corollary:#1}}
\newcommand{\assref}[1]{Assertion~\ref{assertion:#1}}
\newcommand{\asslab}[1]{\label{assertion:#1}}
\newcommand{\thmref}[1]{Theorem~\ref{theorem:#1}}
\newcommand{\thmlab}[1]{\label{theorem:#1}}
\newcommand{\thmsref}[2]{Theorems \ref{theorem:#1} and~\ref{theorem:#2}}
\newcommand{\lemmaref}[1]{Lemma~\ref{lemma:#1}}
\newcommand{\lemmalab}[1]{\label{lemma:#1}}
\newcommand{\propref}[1]{Proposition~\ref{proposition:#1}}
\newcommand{\proplab}[1]{\label{proposition:#1}}
\newcommand{\algoref}[1]{Algorithm~\ref{algorithm:#1}}
\newcommand{\algolab}[1]{\label{algorithm:#1}}
\newcommand{\appref}[1]{App.~\ref{app:#1}}
\newcommand{\applab}[1]{\label{app:#1}}
\newcommand{\secsref}[2]{Secs.~\ref{sec:#1} and~\ref{sec:#2}}
\newcommand{\tablab}[1]{\label{tab:#1}}
\newcommand{\tabref}[1]{Table.~\ref{tab:#1}}
\newcommand{\biblab}[1]{\label{bib:#1}}
\newcommand{\bibref}[1]{[\ref{bib:#1}]}
\newcommand{\conref}[1]{Conjecture~\ref{conjecture:#1}}
\newcommand{\conlab}[1]{\label{conjecture:#1}}
%  Hvilke saetninger, lemmaer etc. og hvordan
%  Paa denne maade faar de alle en faelles nummerering:
% 
%    \newtheorem{thm}{Theorem}[section]
%    \newtheorem{prop}[thm]{Proposition}
%    \newtheorem{lemma}[thm]{Lemma}
%    \newtheorem{cor}[thm]{Corollary}
%    \theoremstyle{definition}
%    \newtheorem{exerc}[thm]{Exercise}
%    \newtheorem{defn}[thm]{Definition}
% \newtheorem{ass}[thm]{Assertion}
%   \newtheorem{exampleee}[thm]{Example}
%    \theoremstyle{remark}
%    \newtheorem{obs}[thm]{Observation}
%    \newtheorem{remark}[thm]{Remark}

%   Paa denne maade faar de hver sin taeller:
%    \theoremstyle{plain}%default
%   \newtheorem{thm}{Theorem}
%   \newtheorem{prop}{Proposition}
%   \newtheorem{lemma}{Lemma}
\newtheorem{cor}{Corollary}
%   \theoremstyle{definition}
%   \newtheorem{defn}{Definition}
%   \newtheorem{exampleee}{Example}
%   \newtheorem{exerc}{Exercise}
\newtheorem{algo}{Algorithm}
  \newtheorem{ass}{Assertion}
\newtheorem{con}{Conjecture}
\newtheorem{saetning}{S�tning}
\newtheorem{paastand}{P�stand}
\newtheorem{bemaerkning}{Bem�rkning}
%   \theoremstyle{remark}
%   \newtheorem{obs}{Observation}
%   \newtheorem{remark}{Remark}
\numberwithin{theorem}{section}
\numberwithin{lemma}{section}
\numberwithin{cor}{section}
\numberwithin{definition}{section}
\numberwithin{equation}{section}
 \numberwithin{example}{section}
  %\numberwithin{prop}{section}
  %\numberwithin{exerc}{section}
  %\numberwithin{obs}{section}
  \numberwithin{remark}{section}


